PartSLIP++: Enhancing Low-Shot 3D Part Segmentation via Multi-View Instance Segmentation and Maximum Likelihood Estimation

Open-world 3D part segmentation is pivotal in diverse applications such as robotics and AR/VR. Traditional supervised methods often grapple with limited 3D data availability and struggle to generalize to unseen object categories. PartSLIP, a recent advancement, has made significant strides in zero- and few-shot 3D part segmentation. This is achieved by harnessing the capabilities of the 2D open-vocabulary detection module, GLIP, and introducing a heuristic method for converting and lifting multi-view 2D bounding box predictions into 3D segmentation masks. In this paper, we introduce PartSLIP++, an enhanced version designed to overcome the limitations of its predecessor. Our approach incorporates two major improvements. First, we utilize a pre-trained 2D segmentation model, SAM, to produce pixel-wise 2D segmentations, yielding more precise and accurate annotations than the 2D bounding boxes used in PartSLIP. Second, PartSLIP++ replaces the heuristic 3D conversion process with an innovative modified Expectation-Maximization algorithm. This algorithm conceptualizes 3D instance segmentation as unobserved latent variables, and then iteratively refines them through an alternating process of 2D-3D matching and optimization with gradient descent. Through extensive evaluations, we show that PartSLIP++ demonstrates better performance over PartSLIP in both low-shot 3D semantic and instance-based object part segmentation tasks. Code released at https://github.com/zyc00/PartSLIP2.

==> tables/ablation_grouping.tex <==
\begin{table}[]
\caption{ablation study about whether using grouping3}
\begin{tabular}{l|lll}
\hline
             & Chair & Kettle & Suitcase \\ \hline
w/ grouping  &       &        &          \\
w/o grouping &       &        &          \\ \hline
\end{tabular}
\end{table}

==> tables/sam_vs_glip_recall.tex <==
\begin{table}[h]
\centering
\caption{This table presents the recall data for three object categories. It compares the method that employs SegmentAnything's 'everything' approach with the method that uses bounding boxes predicted by GLIP as SAM prompts.}
\label{tab:sam_vs_glip_recall}
\begin{tabular}{c|cccc}
\hline
Method &
  Knife &
  Chair &
  Kettle &
  Suitcase \\ \hline
\begin{tabular}[c]{@{}c@{}}GLIP\\ +SAM\end{tabular} &
  58.8 &
  95.5 &
  92.8 &
  75.2 \\ \hline
\begin{tabular}[c]{@{}c@{}}SAM\\ everything\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}74.8\\ (+16.0)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}92.4\\ (-3.1)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}100\\ (+7.2)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}79.5\\ (+4.3)\end{tabular} \\ \hline
\end{tabular}
\end{table}
